A parametric study on the buckling of functionally graded material plates with internal discontinuities using the partition of unity method

In this paper, the effect of local defects, viz., cracks and cutouts on the buckling behaviour of functionally graded material plates subjected to mechanical and thermal load is numerically studied. The internal discontinuities, viz., cracks and cutouts are represented independent of the mesh within the framework of the extended finite element method and an enriched shear flexible 4-noded quadrilateral element is used for the spatial discretization. The properties are assumed to vary only in the thickness direction and the effective properties are estimated using the Mori-Tanaka homogenization scheme. The plate kinematics is based on the first order shear deformation theory. The influence of various parameters, viz., the crack length and its location, the cutout radius and its position, the plate aspect ratio and the plate thickness on the critical buckling load is studied. The effect of various boundary conditions is also studied. The numerical results obtained reveal that the critical buckling load decreases with increase in the crack length, the cutout radius and the material gradient index. This is attributed to the degradation in the stiffness either due to the presence of local defects or due to the change in the material composition.

==> mBuck.tex <==
\paragraph*{Effect of crack} Next, we study the influence of the crack length, the crack orientation, the gradient index and the type of loading on the critical buckling load for a square simply supported FGM plate with thickness $a/h=$ 10 and 100 is studied. \fref{fig:mbuck_nVari_SS2} shows the influence of the gradient index on the critical buckling load for a FGM plate with a horizontal crack with length $d/a=$ 0.4, subjected to uni- and bi-axial compressive loads. It is observed that with increase in gradient index $n$, the critical buckling load decreases for both the uni- and bi-axial compressive loads. This is because of the stiffness degradation due to increase in the metallic volume fraction. \fref{fig:mbuck_caVari_SS2} and Table \ref{tab:mechCrtLoad_Vs_angle_and_Gindex} shows the influence of the crack length and the crack orientation for a square FGM plate subjected to uni- and bi-axial compressive loads. It can be observed that increasing the crack length and the crack orientation decreases the critical buckling load. Further, it is observed that the frequency is lowest for a crack orientation $\theta=$ 90$^\circ$ when the plate is subjected to uni-axial compressive load. When the plate is subjected to bi-axial compressive load, the critical buckling load initially decreases, with further increase in crack orientation, the critical buckling load increases and reaches maximum at $\theta=$90$^\circ$.

% influence of gradiet index on critical buckling load of FGM plates subjected to mechanical loads
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/mbuckUni_nVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/mbuckBi_nVari_SS2}}
\caption{Critical buckling load as a function of gradient index for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads with $a/h=$100 and crack length $c/a$=0.4.}
\label{fig:mbuck_nVari_SS2}
\end{figure}


% influence of crack length on critical buckling load of FGM plates subjected to mechanical loads
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/mbuckUni_caVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/mbuckBi_caVari_SS2}}
\caption{Critical buckling load as a function of crack length $c/a$ for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads.}
\label{fig:mbuck_caVari_SS2}
\end{figure}

% influence of crack orientation, gradient index on critical buckling load of FGM plates subjected to mechanical loads (uni, biaxial)
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{Influence of the crack orientation and the gradient index on the critical buckling load for a simply supported square FGM plates subjected to mechanical loads, viz., uni, biaxial compression with $a/h=$100 and crack length $c/a=$0.4.}
\begin{tabular}{lrrrrrrrr}
\hline
Crack & \multicolumn{8}{c}{gradient index, $n$} \\
\cline{2-9}
Angle,& \multicolumn{2}{c}{0} && \multicolumn{2}{c}{1} && \multicolumn{2}{c}{5}  \\
\cline{2-3}\cline{5-6}\cline{8-9}
$\beta$     & uni   & bi   & & uni   & bi    && uni   & bi \\
\hline
0     & 3.4268 & 1.6729 && 1.5348 & 0.7473 && 1.0749 & 0.5236 \\
30    & 3.3527 & 1.6549 && 1.4962 & 0.7378 && 1.0496 & 0.5177 \\
45    & 3.3141 & 1.6582 && 1.4753 & 0.7391 && 1.0352 & 0.5183 \\
90    & 3.2263 & 1.6729 && 1.4294 & 0.7473 && 1.0044 & 0.5236 \\
\hline
\end{tabular}%
\label{tab:mechCrtLoad_Vs_angle_and_Gindex}%
\end{table}%


%----------- Effect of cutout...
\paragraph*{Effect of cutouts} Next, we study the influence of a centrally located circular cutout on the critical buckling load and critical buckling temperature for a FGM plate. \fref{fig:MechBuck_ab_roaVari} shows the influence of the plate aspect ratio, the gradient index and a centrally located cutout on the critical buckling load when the FGM plate is subjected to a uniaxial compressive load. It can be seen that the combined effect of increasing the gradient index, the cutout radius and the plate aspect ratio is to decrease the critical buckling load. The decrease in the critical load due to the gradient index and the cutout radius can be attributed to the stiffness degradation due to increased metallic volume fraction and due to the presence of a discontinuity, respectively. The influence of the plate aspect ratio is attributed to the geometry effect. \fref{fig:MechBuck_holeRadVari} shows the influence of the centrally located cutout radius and the gradient index on the critical buckling load under two different types of boundary conditions, viz., all edges simply supported and all edges clamped. Here again, the plate is subjected to a uni-axial compressive load along the $y-$ direction. It can be seen that increasing the gradient index decreases the critical buckling load due to increasing metallic volume fraction, whilst, increasing the cutout radius lowers the critical buckling load in the case of simply supported boundary conditions and increases in the case of all edges clamped boundary. The influence of the boundary condition on the critical buckling load can be clearly observed from this study. The influence of randomly located circular cutout on the critical buckling load and the critical buckling temperature is shown in \fref{fig:multi_cut_outs}. A simply supported square FGM plate with $a/h=$ 100 and gradient index, $n=$ 5 is used and is subjected to uni-axial compressive load and nonlinear temperature rise through the thickness of the plate. It can be seen that increasing the number of cutouts, decreases the critical buckling load and the critical buckling temperature. This can be attributed to stiffness degradation due to the presence of cutouts.

% effect of plate aspect ratio on critical buckling load for various gradient index, and center cutout radius
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.75]{./Figures/Mbuck_ab_r0aVari}
\caption{Influence of the plate aspect ratio $a/b$ on the critical buckling load, $\Lambda_{uni} = \frac{N_{xxcr}^o b^2}{\pi^2 D}$, of the FGM plate subjected to uniaxial loading for different gradient index $n$ with a center cutout of radius, $r_o/a=$ 0.1 and $h/b=$ 0.1.}
\label{fig:MechBuck_ab_roaVari}
\end{figure}

% effect of center cutout radius on critical buckling load for various gradient index and boundary conditions
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.75]{./Figures/Mbuck_holeRadVari}
\caption{Variation of the critical buckling load, $\Lambda_{uni} = \frac{N_{xxcr}^o b^2}{\pi^2 D}$ with cutout dimensions for a square FGM plate with $a/h=10$ subjected to uniaxial loading for different gradient index $n$ and boundary conditions.}
\label{fig:MechBuck_holeRadVari}
\end{figure}

==> mechbuck.tex <==
\subsection{Mechanical Buckling}


\subsubsection{Effect of crack length $c/a$, crack orientation $\beta$ and gradient index $n$}
The influence of the crack length $c/a$, crack orientation $\beta$ and the gradient index $n$ on the critical buckling load for a simply supported square FGM plate with thickness $a/h=$ 10 is shown.

It is observed that as the crack length increases, the critical buckling load decreases for both uni-axial and bi-axial compressive loads. This is attributed to the fact that as the crack length increases, the local flexibility increases and thus decreases the critical buckling load. The effect of the gradient index $n$ is shown in Table \ref{table:SS_MechBuck_theta}. With increase in the gradient index $n$, the critical buckling load decreases. This is because of the stiffness degradation due to increase in the metallic volume fraction. It is observed that the combined effect of increasing the crack length and the gradient index is to decrease the critical buckling load. It can also be seen from Table \ref{table:SS_MechBuck_theta} that for uni-axial compressive load, the critical buckling load is minimum when the crack orientation $\theta=$90$^\circ$ (i.e, crack is perpendicular to the loading direction), whilst for the bi-axial compressive stress, the critical buckling load is minimum for a crack orientation $\theta=$45$^\circ$.

% influence of crack orientation, gradient index on critical buckling load of FGM plates subjected to mechanical loads (uni, biaxial)
\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Influence of the crack orientation and the gradient index on the critical buckling load for a simply supported square FGM plates subjected to mechanical loads, viz., uni, biaxial with $a/h=$10 and crack length $c/a=$0.4.}
\centering
\begin{tabular}{cccccc}
\hline 
$\beta$ &  & \multicolumn{4}{c}{Gradient index k} \\
\cline{3-6}
&  & 0 & 2 & 5 & 10\\
\hline
\multirow{2}{*}{0$^\circ$} & $\lambda_{\rm{uni}}$ & 3.4268 & 1.3021 & 1.0749 & 0.9261 \\
& $\lambda_{\rm{bi}}$ & 1.6729 & 0.6337 & 0.5239 & 0.4516 \\
\cline{2-6}
\multirow{2}{*}{30$^\circ$} & $\lambda_{\rm{uni}}$ & 3.3527 & 1.2694 & 1.0496 & 0.9055 \\
& $\lambda_{\rm{bi}}$ & 1.6549 & 0.6258 & 0.5177 & 0.4467 \\
\cline{2-6}
\multirow{2}{*}{45$^\circ$} & $\lambda_{\rm{uni}}$ & 3.3141 & 1.2510 & 1.0352 & 0.8938 \\
& $\lambda_{\rm{bi}}$ & 1.6582 & 0.6268 & 0.5183 & 0.4473 \\
\cline{2-6}
\multirow{2}{*}{90$^\circ$} & $\lambda_{\rm{uni}}$ & 3.2263 & 1.2113 & 1.0044 & 0.8686 \\
& $\lambda_{\rm{bi}}$ & 1.6729 & 0.6337 & 0.5236 & 0.4516 \\
\hline
\end{tabular}
\label{table:SS_MechBuck_theta}
\end{table}

% pictorial representation of the above table
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/mbuckUni_caVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/mbuckBi_caVari_SS2}}
\caption{Critical buckling load as a function of crack orientation for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads with $a/h=$10 and crack length $c/a$=0.4.}
\label{}
\end{figure}

% pictorial representation of the above table
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{mbuckUni_nVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{mbuckBi_nVari_SS2}}
\caption{Critical buckling load as a function of gradient index for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads with $a/h=$100 and crack length $c/a$=0.4.}
\label{}
\end{figure}

% variation of critical buckling load with crack length, plate thickness and plate aspect ratio
%\begin{figure}[htpb]
%\centering
%\subfigure[Uni-axial]{\includegraphics[scale=0.75]{mbuckUni_caVari}}
%\subfigure[Bi-axial]{\includegraphics[scale=0.75]{mbuckBi_caVari}}
%\caption{Variation of critical bucking load for a simply supported FGM plate for various plate thickness, viz., $a/h$= 10, 100 and gradient index $n=$0,5.}
%\label{fig:cambuck}
%\end{figure}


% effect of crack location on the critical buckling load
\subsubsection{Effect of crack location}
Next, the influence of the crack location on the critical buckling load of a simply supported square FGM plate (gradient index, $n=$ 2) subjected to bi-axial compressive load for think plate $a/h=$ 100 and crack length $c/a=$0.4 is studied. The results are depicted in \fref{fig:mechBuckCrkLoc} and it is observed that the critical buckling load is lowest when the crack is situated at the center of the square plate. As the crack move from the edges of the plate towards the center of the plate, the critical buckling load monotonically decreases. The critical buckling load is maximum when the crack is located at the corner.
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.75]{./Figures/mbuck_crkLoc3d}}
\subfigure[]{\includegraphics[scale=0.75]{./Figures/mbuck_crkLoc}}
\caption{Effect of crack location on the critical buckling load $(\lambda_{\rm{bi}}$ for a simply supported square FGM plate (gradient index, $n=$ 2) subjected to bi-axial compressive load with $a/h=$100, $c/a$=0.4 and the crack orientation, $\theta$ is taken to be 0.}
\label{fig:mechBuckCrkLoc}
\end{figure}


==> platewcrack.tex <==
\subsection{Plate with cracks}

%----------------------------------------------------
%		EFFECT OF CENTER CRACK
%----------------------------------------------------
\paragraph*{Effect of center crack}
The influence of the crack length $(c/a)$ on the critical buckling load for a simply supported square FGM plate with thickness $a/h=$ 100, 10 and gradient index $n=$ 0, 5 under uni-axial and bi-axial compressive loading is shown in \fref{fig:mbuck_caVari_SS2}. Numerical values for critical buckling load has been produced in Table \ref{tab:mechCrtLoad_Vs_angle_and_Gindex} for different crack orientation and gradient index under uniaxial and biaxial compressive loading.
It is been observed that as the crack length increases, the critical buckling load decreases for both uni-axial and bi-axial compressive loads. This is attributed to the fact that as the crack length increases, the local flexibility increases and thus decreases the critical buckling load. And the effect of crack length on critical buckling load is more pronounced in the case of isotropic plate ($n=$0) than graded plate ($n=$5) as can be seen from the slope of the curves in \fref{fig:mbuck_caVari_SS2}.

Similar study has been made on the effect of crack length $c/a$ on critical buckling load in thermal loading with different thickness $a/h=$ 100, 10 and gradient index $n=$ 0, 5 under linear and non-linear through thickness temperature variation as shown in  \fref{fig:thbuck_caVari_SS2}. The effect is similar, with increased crack length critical buckling load is decreased . Numerical values of critical thermal load for various crack orientation, $\theta$ and gradient index, $n$ has been produced in Table \ref{tab:thCrtLoad_Vs_angle_and_Gindex} under both linear and non-linear through thickness temperature variation.

% influence of crack orientation, gradient index on critical buckling load of FGM plates subjected to mechanical loads (uni, biaxial)
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{Influence of the crack orientation and the gradient index on the critical buckling load for a simply supported square FGM plates subjected to mechanical loads, viz., uni, biaxial compression with $a/h=$100 and crack length $c/a=$0.4.}
\begin{tabular}{lrrrrrrrr}
\hline
Crack & \multicolumn{8}{c}{gradient index, $n$} \\
\cline{2-9}
Angle,& \multicolumn{2}{c}{0} && \multicolumn{2}{c}{1} && \multicolumn{2}{c}{5}  \\
\cline{2-3}\cline{5-6}\cline{8-9}
$\beta$     & uni   & bi   & & uni   & bi    && uni   & bi \\
\hline
0     & 3.4268 & 1.6729 && 1.5348 & 0.7473 && 1.0749 & 0.5236 \\
30    & 3.3527 & 1.6549 && 1.4962 & 0.7378 && 1.0496 & 0.5177 \\
45    & 3.3141 & 1.6582 && 1.4753 & 0.7391 && 1.0352 & 0.5183 \\
90    & 3.2263 & 1.6729 && 1.4294 & 0.7473 && 1.0044 & 0.5236 \\
\hline
\end{tabular}%
\label{tab:mechCrtLoad_Vs_angle_and_Gindex}%
\end{table}%


% influence of crack length on critical buckling load of FGM plates subjected to mechanical loads
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/mbuckUni_caVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/mbuckBi_caVari_SS2}}
\caption{Critical buckling load as a function of crack length $c/a$ for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads.}
\label{fig:mbuck_caVari_SS2}
\end{figure}


% influence of crack orientation, gradient index on critical buckling load of FGM plates subjected to thermal loads (linear, nonlinear)
\begin{table}[htbp]
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Influence of the crack orientation and the gradient index on the critical buckling load for a simply supported square FGM plates subjected to thermal loads, viz., through thickness temperature variation with $a/h=$100 and crack length $c/a=$0.4.}
\begin{tabular}{rrrrrrrrr}
\hline
Crack & \multicolumn{8}{c}{gradient index, $n$} \\
\cline{2-9}
Angle, & \multicolumn{2}{c}{0} & & \multicolumn{2}{c}{1} & & \multicolumn{2}{c}{5}  \\
\cline{2-3}\cline{5-6}\cline{8-9}
$\beta$ & T$_{_L}$   & T$_{_{NL}}$   & & T$_{_L}$   & T$_{_{NL}}$   & & T$_{_L}$   & T$_{_{NL}}$ \\
\hline
0     & 19.0289 & 19.0289 && 3.2929 & 4.5708 && 3.3978 & 4.2494 \\
30    & 18.4965 & 18.4965 && 3.0552 & 4.2410 && 3.1570 & 3.9483 \\
45    & 18.5432 & 18.5432 && 3.0791 & 4.2741 && 3.1689 & 3.9631 \\
90    & 19.0289 & 19.0289 && 3.2929 & 4.5708 && 3.3978 & 4.2494 \\
\hline
\end{tabular}%
\label{tab:thCrtLoad_Vs_angle_and_Gindex}%
\end{table}%



% influence of crack length on critical buckling load of FGM plates subjected to mechanical loads 
\begin{figure}[htpb]
\centering
\subfigure[Thick plate]{\includegraphics[scale=0.75]{./Figures/thbuck_SS2_thick_caVari}}
\subfigure[Thin Plate]{\includegraphics[scale=0.75]{./Figures/thbuck_SS2_thin_caVari}}
\caption{Critical buckling load as a function of crack length $c/a$ for a simply supported square FGM plate with thickness $a/h=$ 100 and 10 subjected to linear and non-linear through thickness temperature variation.}
\label{fig:thbuck_caVari_SS2}
\end{figure}


%\subsubsection{Effect of center crack on critical buckling load with different gradient index $(n)$.}

\fref{fig:mbuck_nVari_SS2} shows the effect of gradient index on the critical buckling load with different crack orientation. It can be seen that there is is a drastic reduction in the critical buckling as the material goes from isotropic to functionally graded. This is due to the fact that higher gradient index means the plate is more metallic which make it less stiff and causes reduction in critical buckling load. Similar result has been observed in the case of thermal loading as can be seen from the \fref{fig:thbuck_nVari_SS2}


% influence of gradiet index on critical buckling load of FGM plates subjected to mechanical loads
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/mbuckUni_nVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/mbuckBi_nVari_SS2}}
\caption{Critical buckling load as a function of gradient index for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads with $a/h=$100 and crack length $c/a$=0.4.}
\label{fig:mbuck_nVari_SS2}
\end{figure}


% influence of gradient index on critical buckling load of FGM plates subjected to thermal loads
\begin{figure}[htpb]
\centering
\subfigure[Linear temperature variation]{\includegraphics[scale=0.75]{./Figures/thbuckLin_nVari_SS2}}
\subfigure[Non-linear temperature variation]{\includegraphics[scale=0.75]{./Figures/thbuckNlin_nVari_SS2}}
\caption{Critical buckling load as a function of gradient index for a simply supported square FGM plate subjected to linear and non-linear through thickness temperature variation with $a/h=$100 and crack length $c/a$=0.4.}
\label{fig:thbuck_nVari_SS2}
\end{figure}

%------------------------------------------------------------
%			EFFECT OF MULTIPLE CRACKS
%------------------------------------------------------------
\paragraph{Effect of multiple cracks}

In this section we will study the effect of multiple cracks of different length and orientation spread throughout the plate. We will increase the number of crack in the successive steps and study the influence on the critical buckling load. One point to be noted here is that though we are placing more number of cracks in the successive steps but we are keeping the previous cracks intact. The study has been made using a square plate with all edges simply supported, thickness $a/h=$ 100 and gradient index $n=$ 1 under uni-axial compressive loading. \fref{fig:multi_crack} shows that there is a steady decrease in the critical buckling load upon increasing the number of cracks.

 Similar study has been made for the same plate under thermal loading with through thickness linear variation of temperature. \fref{fig:multi_crack} shows that in this case also the critical buckling temperature decreases as the number of crack is increased.
 
 
\begin{figure}[htpb]
\centering
\subfigure[Mechancial]{\includegraphics[scale=0.75]{./Figures/mech_multi_crack}}
\subfigure[Thermal]{\includegraphics[scale=0.75]{./Figures/th_multi_crack}}
\caption{Critical buckling load as a function of number of cracks for a simply supported square FGM plate with $a/h=$100 and $n=$1 subjected to (a) uni-axial compressive loading (b) linear through thickness temperature variation.}
\label{fig:multi_crack}
\end{figure}

==> platewcutout.tex <==
\subsection{Plate with cutouts}

%-----------------------------------------------
%		CIRCULAR CUTOUT
%----------------------------------------------
In this section we will study the effect of material discontinuity in the form of circular cutouts on critical buckling load of FGM plates under different cutout size, plate aspect ratio and gradient index. 


\fref{fig:MechBuck_ab_roaVari} shows the influence of cutout on critical buckling load for an isotropic(n=0 pure ZrO$_2$) and FGM(n=5) plate under different plate aspect ratio similar trend trend has been observed for plates with all edges are clamped. From the figure it is clear that having a cutout in the plate reduces the critical buckling load drastically. Increase in critical buckling load beyond some specific cutout radius is due to the fact that XXXXXXXXXXXXXXXX .
% SS, FGM plate, a/h=100, r/a=0.1, critical buckling load - mechanical uniaxial


% effect of plate aspect ratio on critical buckling load for various gradient index, and center cutout radius
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.75]{./Figures/Mbuck_ab_r0aVari}
\caption{Influence of the plate aspect ratio $a/b$ on the critical buckling load, $\Lambda_{uni} = \frac{N_{xxcr}^o b^2}{\pi^2 D}$, of the FGM plate subjected to uniaxial loading for different gradient index $n$ with a center cutout of radius, $r_o/a=$ 0.1 and $h/b=$ 0.1.}
\label{fig:MechBuck_ab_roaVari}
\end{figure}


% effect of center cutout radius on critical buckling load for various gradient index and boundary conditions
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.75]{./Figures/Mbuck_holeRadVari}
\caption{Variation of the critical buckling load, $\Lambda_{uni} = \frac{N_{xxcr}^o b^2}{\pi^2 D}$ with cutout dimensions for a square FGM plate with $a/h=10$ subjected to uniaxial loading for different gradient index $n$ and boundary conditions.}
\label{fig:MechBuck_ab_roaVari}
\end{figure}


\paragraph*{Effect of multiple cutouts}
Effect of multiple cutouts of different radius spread throughout the plate has been studied in this section. \fref{fig:multi_cutouts_plate} shows a typical plate with multiple cutouts. Here we will increase the number of cutouts in the successive steps and study the influence on critical buckling load. Like in the case of multiple cracks (section \ref{multi_crack}) one point to be noted here also that though we are placing more number of cutouts in the successive steps but we are keeping the previous cutouts intact. The study has been made using a square plate with all edges simply supported, thickness $a/h=$ 100 and gradient index $n=$ 5 under uni-axial compressive loading. \fref{fig:multi_cut_outs} shows that there is a steady decrease in the critical buckling load upon increasing the number of cutouts.

 Similar study has been made for the same plate under thermal loading with through thickness nonlinear variation of temperature. \fref{fig:multi_cut_outs} shows that in this case also the critical buckling temperature decreases as the number of cutouts is increased.

% typical plate with multiplae cutouts. 
\begin{figure}[htpb]
\centering
\includegraphics[scale=0.75]{./Figures/multi_cutouts_plate}
\caption{Typical plate with multiple cutouts.}
\label{fig:multi_cutouts_plate}
\end{figure}

\begin{figure}[htpb]
\centering
\subfigure[Mechancial]{\includegraphics[scale=0.75]{./Figures/mech_multi_cutouts}}
\subfigure[Thermal]{\includegraphics[scale=0.75]{./Figures/th_multi_cutouts}}
\caption{Critical buckling load as a function of number of cutouts for a simply supported square FGM plate with $a/h=$100 and $n=$5 subjected to (a) uni-axial compressive loading (b) nonlinear through thickness temperature variation.}
\label{fig:multi_cut_outs}
\end{figure}

==> tBuck.tex <==
\paragraph*{Effect of crack}

% influence of crack orientation, gradient index on critical buckling load of FGM plates subjected to thermal loads (linear, nonlinear)
\begin{table}[htbp]
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Influence of the crack orientation and the gradient index on the critical buckling load for a simply supported square FGM plates subjected to thermal loads, viz., through thickness temperature variation with $a/h=$100 and crack length $c/a=$0.4.}
\begin{tabular}{rrrrrrrrr}
\hline
Crack & \multicolumn{8}{c}{gradient index, $n$} \\
\cline{2-9}
Angle, & \multicolumn{2}{c}{0} & & \multicolumn{2}{c}{1} & & \multicolumn{2}{c}{5}  \\
\cline{2-3}\cline{5-6}\cline{8-9}
$\beta$ & T$_{_L}$   & T$_{_{NL}}$   & & T$_{_L}$   & T$_{_{NL}}$   & & T$_{_L}$   & T$_{_{NL}}$ \\
\hline
0     & 19.0289 & 19.0289 && 3.2929 & 4.5708 && 3.3978 & 4.2494 \\
30    & 18.4965 & 18.4965 && 3.0552 & 4.2410 && 3.1570 & 3.9483 \\
45    & 18.5432 & 18.5432 && 3.0791 & 4.2741 && 3.1689 & 3.9631 \\
90    & 19.0289 & 19.0289 && 3.2929 & 4.5708 && 3.3978 & 4.2494 \\
\hline
\end{tabular}%
\label{tab:thCrtLoad_Vs_angle_and_Gindex}%
\end{table}%


% influence of gradient index on critical buckling load of FGM plates subjected to thermal loads
\begin{figure}[htpb]
\centering
\subfigure[Linear temperature variation]{\includegraphics[scale=0.75]{./Figures/thbuckLin_nVari_SS2}}
\subfigure[Non-linear temperature variation]{\includegraphics[scale=0.75]{./Figures/thbuckNlin_nVari_SS2}}
\caption{Critical buckling load as a function of gradient index for a simply supported square FGM plate subjected to linear and non-linear through thickness temperature variation with $a/h=$100 and crack length $c/a$=0.4.}
\label{fig:thbuck_nVari_SS2}
\end{figure}

==> thereferences.tex <==
\begin{thereferences}{90}

\bibitem{Reddy_FGM_1998}Reddy J N. 
Thermomechanical analysis of functionally graded cylinders and plates.
\textit{Journal of Thermal Stresses}
\textbf{Volume 21, Issue 6, 593-626, 1998}




Thermal buckling of functionally graded plates based on higher order theory. R Javaheri, M R eslami. Journal of Thermal Stresses[Volume 25, Issue 7,603-625, 2002]


Free vibration analysis of Functionally Graded Plates with Multiple Circular and Non-circular Cutouts. J Maziar, R Iman. Chinese Journal of Mechanicsl Engineering[Vol 24, No 6, 2011]


\end{thereferences}

==> thermbuck.tex <==
\subsection{Thermal Buckling}

\subsubsection{Effect of crack length $c/a$, crack orientation $\beta$ and gradient index $n$}
The influence of the crack length $c/a$, crack orientation $\beta$ and the gradient index $n$ on the critical buckling load for a simply supported square FGM plate with different thickness $a/h=$ 10 and 100 is shown.

It is observed that as the crack length increases, the critical buckling load decreases for both uni-axial and bi-axial compressive loads. This is attributed to the fact that as the crack length increases, the local flexibility increases and thus decreases the critical buckling load. The effect of the gradient index $n$ is shown in Table \ref{table:SS_MechBuck_theta}. With increase in the gradient index $n$, the critical buckling load decreases. This is because of the stiffness degradation due to increase in the metallic volume fraction. It is observed that the combined effect of increasing the crack length and the gradient index is to decrease the critical buckling load. It can also be seen from Table \ref{table:SS_MechBuck_theta} that for uni-axial compressive load, the critical buckling load is minimum when the crack orientation $\theta=$90$^\circ$ (i.e, crack is perpendicular to the loading direction), whilst for the bi-axial compressive stress, the critical buckling load is minimum for a crack orientation $\theta=$45$^\circ$.

% influence of crack orientation, gradient index on critical buckling load of FGM plates subjected to mechanical loads (uni, biaxial)
\begin{table}[htpb]
\renewcommand\arraystretch{1.5}
\caption{Influence of the crack orientation and the gradient index on the critical buckling load for a simply supported square FGM plates subjected to mechanical loads, viz., uni, biaxial with $a/h=$10 and crack length $c/a=$0.4.}
\centering
\begin{tabular}{cccccc}
\hline 
$\beta$ &  & \multicolumn{4}{c}{Gradient index k} \\
\cline{3-6}
&  & 0 & 2 & 5 & 10\\
\hline
\multirow{2}{*}{0$^\circ$} & $\lambda_{\rm{uni}}$ & 3.4268 & 1.3021 & 1.0749 & 0.9261 \\
& $\lambda_{\rm{bi}}$ & 1.6729 & 0.6337 & 0.5239 & 0.4516 \\
\cline{2-6}
\multirow{2}{*}{30$^\circ$} & $\lambda_{\rm{uni}}$ & 3.3527 & 1.2694 & 1.0496 & 0.9055 \\
& $\lambda_{\rm{bi}}$ & 1.6549 & 0.6258 & 0.5177 & 0.4467 \\
\cline{2-6}
\multirow{2}{*}{45$^\circ$} & $\lambda_{\rm{uni}}$ & 3.3141 & 1.2510 & 1.0352 & 0.8938 \\
& $\lambda_{\rm{bi}}$ & 1.6582 & 0.6268 & 0.5183 & 0.4473 \\
\cline{2-6}
\multirow{2}{*}{90$^\circ$} & $\lambda_{\rm{uni}}$ & 3.2263 & 1.2113 & 1.0044 & 0.8686 \\
& $\lambda_{\rm{bi}}$ & 1.6729 & 0.6337 & 0.5236 & 0.4516 \\
\hline
\end{tabular}
\label{table:SS_MechBuck_theta}
\end{table}

% pictorial representation of the above table
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/thbuck_SS2_thick_caVari}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/thbuck_SS2_thin_caVari}}
\caption{Critical buckling load as a function of crack orientation for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads with $a/h=$10 and crack length $c/a$=0.4.}
\label{fig:thbuckUniBi_caVari_SS2}
\end{figure}

% pictorial representation of the above table
\begin{figure}[htpb]
\centering
\subfigure[Uni-axial]{\includegraphics[scale=0.75]{./Figures/thbuckLin_nVari_SS2}}
\subfigure[Bi-axial]{\includegraphics[scale=0.75]{./Figures/thbuckNlin_nVari_SS2}}
\caption{Critical buckling load as a function of gradient index for a simply supported square FGM plate subjected to uni-axial and bi-axial compressive loads with $a/h=$100 and crack length $c/a$=0.4.}
\label{}
\end{figure}

% variation of critical buckling load with crack length, plate thickness and plate aspect ratio
%\begin{figure}[htpb]
%\centering
%\subfigure[Uni-axial]{\includegraphics[scale=0.75]{mbuckUni_caVari}}
%\subfigure[Bi-axial]{\includegraphics[scale=0.75]{mbuckBi_caVari}}
%\caption{Variation of critical bucking load for a simply supported FGM plate for various plate thickness, viz., $a/h$= 10, 100 and gradient index $n=$0,5.}
%\label{fig:cambuck}
%\end{figure}


% effect of crack location on the critical buckling load
\subsubsection{Effect of crack location}
Next, the influence of the crack location on the critical buckling load of a simply supported square FGM plate (gradient index, $n=$ 2) subjected to bi-axial compressive load for think plate $a/h=$ 100 and crack length $c/a=$0.4 is studied. The results are depicted in \fref{fig:mechBuckCrkLoc} and it is observed that the critical buckling load is lowest when the crack is situated at the center of the square plate. As the crack move from the edges of the plate towards the center of the plate, the critical buckling load monotonically decreases. The critical buckling load is maximum when the crack is located at the corner.
\begin{figure}[htpb]
\centering
\subfigure[]{\includegraphics[scale=0.75]{./Figures/mbuck_crkLoc3d}}
\subfigure[]{\includegraphics[scale=0.75]{./Figurs/mbuck_crkLoc}}
\caption{Effect of crack location on the critical buckling load $(\lambda_{\rm{bi}}$ for a simply supported square FGM plate (gradient index, $n=$ 2) subjected to bi-axial compressive load with $a/h=$100, $c/a$=0.4 and the crack orientation, $\theta$ is taken to be 0.}
\label{fig:mechBuckCrkLoc}
\end{figure}

